A Purely-Reactive Manipulability-Maximising Motion Controller

We present a novel approach to controlling the instantaneous velocity of a robot end-effector that is able to simultaneously maximise manipulability and avoid joint limits. It operates on non-redundant and redundant robots, which is achieved by adding artificial redundancy in the form of controlled path deviation. We formulate the problem as a quadratic programme and provide an open-source Python implementation that provides solutions in just a few milliseconds. It accepts a robot model expressed using URDF or Denavit-Hartenberg parameterisation. We compare our method to previous work in simulation and on a physical robot.

==> 9_dot_m.tex <==

The manipulability Jacobian is obtained by taking the time derivative of (\ref{m:man1}) and applying the chain rule

\begin{align} \label{m:man22}
    \frac{\mathrm{d} \ m(t)}
         {\mathrm{d} t} = 
    \dfrac{1}
          {2m(t)} 
    \frac{\mathrm{d} \ \mbox{det} \left( \matfn{J}{\vec{q}} \matfn{J}{\vec{q}}^\top \right)}
         {\mathrm{d} t} 
\end{align}
%
where  $\mbox{det} \left( \matfn{J}{\vec{q}} \matfn{J}{\vec{q}}^\top \right)$ is a scalar function of a vector. Jacobi's formula expresses the derivative of the determinant of a matrix \cite{jacobi}


\begin{align} \label{m:jacobi}
    \dfrac{\mathrm{d} \ \mbox{det} (\matfn{A}{x})}
          {\mathrm{d} x}
    &= \mbox{tr} 
    \left( 
        \mbox{adj} \left( \matfn{A}{x} \right) 
        \dfrac{\mathrm{d} \matfn{A}{x}}
              {\mathrm{d} x} 
    \right) \nonumber \\
    &= \mbox{det} (\matfn{A}{x}) \ \mbox{tr} 
    \left( 
        \matfn{A}{x}^{-1} \dfrac{\mathrm{d} \matfn{A}{x}}
                                {\mathrm{d} x} 
    \right)
\end{align}
%
where $\mbox{adj}(\mat{A}) = \mbox{det}(\mat{A})\mat{A}^{-1}$ is the adjugate of a matrix, and $\mbox{tr}(\cdot)$ is the trace of a matrix. Using (\ref{m:jacobi}) to expand the rightmost term of (\ref{m:man22}) gives

\begin{equation} \label{m:man3}
    \dfrac{\mathrm{d} \left( \mbox{det} (\mat{J}\mat{J}^\text{T}) \right) }
          {\mathrm{d} t}
    = \mbox{det} \left( \mat{J}\mat{J}^\text{T} \right) 
    \mbox{tr} \left( 
        (\mat{J}\mat{J}^\text{T})^{-1} \dfrac{\mathrm{d} \mat{J}\mat{J}^\text{T}}
                                             {\mathrm{d}t}
    \right).
\end{equation}

Additionally, using the product rule to expand the remaining derivative in (\ref{m:man3})

\begin{align*}
    \dfrac{\mathrm{d} \left( \mbox{det} (\mat{J}\mat{J}^\text{T}) \right) }
          {\mathrm{d} t}
    &=  \mbox{det} \left( \mat{J}\mat{J}^\text{T} \right) 
    \text{tr} \left( 
        (\mat{J}\mat{J}^\text{T})^{-1} 
        ( \mat{J} \dmat{J^\text{T}} + \dmat{J} \mat{J}^\text{T} )
    \right)
\end{align*}
%
where $\dmat{J}$ is the time derivative of $\mat{J}$. Using the property $\dot{(\mat{J}^\top)} = (\dmat{J})^\top$, the trace product property, and the trace cyclic property, this can be simplified to

\begin{align} \label{m:man4}
    \dfrac{\mathrm{d} \left( \mbox{det} (\mat{J}\mat{J}^\text{T}) \right) }
          {\mathrm{d} t}
    &=  
    \text{det} \left( \mat{J}\mat{J}^\text{T} \right) \times \nonumber \\
    & \qquad \quad \mbox{tr} \left( 
        \dmat{J} \mat{J}^\text{T} (\mat{J}\mat{J}^\text{T})^{-1} +
        \dmat{J} \mat{J}^\text{T} (\mat{J}\mat{J}^\text{T})^{-1}
    \right) \nonumber \\ 
    &=  
    2 \ \text{det} \left( \mat{J}\mat{J}^\text{T} \right) 
    \mbox{tr} \left( 
        \dmat{J} \mat{J}^\text{T} (\mat{J}\mat{J}^\text{T})^{-1} 
    \right).
\end{align}

Substituting (\ref{m:man4}) back into (\ref{m:man22}) yields

\begin{align} \label{m:man5}
    \dot{m} &= \dfrac{1}
                     {2m(t)}2 \ 
    \mbox{det} \left( \mat{J}\mat{J}^\top \right) 
    \mbox{tr} \left( 
        \dmat{J} \mat{J}^\top (\mat{J}\mat{J}^\top)^{-1} 
    \right) \nonumber \\
    &= \sqrt{ \mbox{det} \left( \mat{J}\mat{J}^\top \right)} \ \ 
    \mbox{tr} \left( 
        \dmat{J} \mat{J}^\top (\mat{J}\mat{J}^\top)^{-1} 
    \right) \nonumber \\
    &= m \ 
    \mbox{tr} \left( 
        \dmat{J} \mat{J}^\top (\mat{J}\mat{J}^\top)^{-1} 
    \right)
\end{align}
%
where $m$ is defined in (\ref{m:man1}), and $\dmat{J}$ is the time derivative of the manipulator Jacobian. Using the chain rule, (\ref{m:man5}) becomes

\begin{align} \label{m:man6}
    \frac{\mathrm{d} \ \matfn{J}{\vec{q}(t)}}
         {\mathrm{d} t} 
    &= 
    \frac{\partial \matfn{J}{\vec{q}}}
         {\partial \vec{q}} 
    \frac{\mathrm{d} \vec{q}(t)}
         {\mathrm{d} t} \nonumber \\
    &= 
    \sum_{i=1}^n \frac{\partial \matfn{J}{\vec{q}}}
                      {\partial q_i}
    \dvec{q}_i  \nonumber \\
    &=
    \sum_{i=1}^n \matfn{H_i}{\vec{q}} \dvec{q}_i \\
    &= 
    \matfn{H}{\vec{q}} \dvec{q} \nonumber
\end{align}
%
where $\matfn{H}{\vec{q}} \in \R^{6 \times n \times n}$ is the manipulator Hessian. Substituting the result from (\ref{m:man6}) into (\ref{m:man5}) we obtain

\begin{align} \label{m:man7}
    \dot{m}
    &= 
    m \ 
    \mbox{tr} \left( 
        \left( \sum_{i=1}^n \mat{H_i} \dvec{q}_i \right)
        \mat{J}^\top (\mat{J}\mat{J}^\top)^{-1} 
    \right) \nonumber \\
    &=
    m \ 
    \sum_{i=1}^n \left(
        \dvec{q}_i \ \mbox{tr} \left(
            \mat{H_i} \mat{J}^\top (\mat{J}\mat{J}^\top)^{-1} 
        \right)
    \right).
\end{align}

Using the relationship $\mat{B}^\top\mat{A}^\top = (\mat{A}\mat{B})^\top$, (\ref{m:man7}) becomes

\begin{align} \label{m:man8}
    \dot{m}
    &=
    m \ 
    \sum_{i=1}^k \left(
        \dvec{q}_i \ \mbox{tr} \left(
            (\mat{J} \mat{H_i}^\top)^\top (\mat{J}\mat{J}^\top)^{-1} 
        \right)
    \right).
\end{align}

Furthermore, using the relationship 

\begin{equation*}
    \mbox{tr}(\mat{A}^\top \mat{B}) = \mbox{vec}(\mat{A})^\top \mbox{vec}(\mat{B}), 
\end{equation*}
%
where the vector operation $\mbox{vec}(\cdot) : \R^{a \times b} \rightarrow \R^{ab}$ vectorises a matrix into a vector, (\ref{m:man8}) becomes

\begin{align} \label{m:man99}
    \dot{m}
    &=
    m \
    \sum_{i=1}^n \left(
        \dvec{q}_i \ 
        \mbox{vec} \left(
            \mat{J} \mat{H_i}^\top
        \right)^\top
        \mbox{vec} \left(
            (\mat{J}\mat{J}^\top)^{-1}
        \right)
    \right) \nonumber \\
    &=
    \sum_{i=1}^n \left(
        \dvec{q}_i \ 
        m \
        \mbox{vec} \left(
            \mat{J} \mat{H_i}^\top
        \right)^\top
        \mbox{vec} \left(
            (\mat{J}\mat{J}^\top)^{-1}
        \right)
    \right) \nonumber \\
    &=
    \begin{pmatrix}
        \dvec{q}_1 \ \ \hdots \ \ \dvec{q}_n
    \end{pmatrix}
    \begin{pmatrix}
        m \ \mbox{vec} \left( \mat{J} \mat{H_1}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
        m \ \mbox{vec} \left( \mat{J} \mat{H_2}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
        \vdots \\
        m \ \mbox{vec} \left( \mat{J} \mat{H_n}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
    \end{pmatrix} \nonumber \\
    &=
    \dvec{q}^\top \ \vec{M} \nonumber \\
    &=
    \vec{M}^\top \ \dvec{q}
\end{align}
%
where

\begin{equation} \label{m:man110}
    \vec{M}
    =
    \begin{pmatrix}
        m \ \mbox{vec} \left( \mat{J} \mat{H_1}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
        m \ \mbox{vec} \left( \mat{J} \mat{H_2}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
        \vdots \\
        m \ \mbox{vec} \left( \mat{J} \mat{H_n}^\top \right)^\top 
        \mbox{vec} \left( (\mat{J}\mat{J}^\top)^{-1} \right) \\
    \end{pmatrix}
\end{equation}
%
is the manipulability Jacobian with $\vec{M}^\top \in \R^n$.
